Sublinear Time Hypergraph Sparsification via Cut and Edge Sampling Queries

The problem of sparsifying a graph or a hypergraph while approximately preserving its cut structure has been extensively studied and has many applications. In a seminal work, Bencz\'ur and Karger (1996) showed that given any $n$-vertex undirected weighted graph $G$ and a parameter $\varepsilon \in (0,1)$, there is a near-linear time algorithm that outputs a weighted subgraph $G'$ of $G$ of size $\tilde{O}(n/\varepsilon^2)$ such that the weight of every cut in $G$ is preserved to within a $(1 \pm \varepsilon)$-factor in $G'$. The graph $G'$ is referred to as a {\em $(1 \pm \varepsilon)$-approximate cut sparsifier} of $G$. Subsequent recent work has obtained a similar result for the more general problem of hypergraph cut sparsifiers. However, all known sparsification algorithms require $\Omega(n + m)$ time where $n$ denotes the number of vertices and $m$ denotes the number of hyperedges in the hypergraph. Since $m$ can be exponentially large in $n$, a natural question is if it is possible to create a hypergraph cut sparsifier in time polynomial in $n$, {\em independent of the number of edges}. We resolve this question in the affirmative, giving the first sublinear time algorithm for this problem, given appropriate query access to the hypergraph.

==> 1 <==
\section{Sublinear Time Cut Sparsification with Cut Size and Pair Neighbor Queries}
\label{sec:ONTWO}

In this section, we show that cut edge queries can be simulated by a $\poly(n)$ number of cut size queries (oracle $\OVA$) and pair neighbor queries (oracle $\ONTWO$), establishing that cut size query oracle and pair neighbor query oracle are also sufficient to compute a $(1 \pm \eps)$-approximate cut sparsifier in $\poly(n)$ time. 

Given a pair of vertices $u$ and $v$, let $E(\{u,v\})$ be the set of edges that contain both $u$ and $v$. We first show how to approximate $|E(\{u,v\})|$ to within a factor of $(1\pm \eps)$ with probability $1-\xi$, for some small $\xi$. Note that we can compute $2 \Delta_{\{u,v\}}(\{u\}) = |E(\{u,v\})| + |E \cap \{u,v\}|$, where $|E\cap \{u,v\}|$ is the number of copies of the edge $\{u,v\}$. We now describe an algorithm to approximate $|E(\{u,v\})|$:

\begin{algorithm}[H] \label{alg:pair}
\SetAlgoLined
	\SetKwInOut{Input}{Input}\SetKwInOut{Output}{Output}

	\Input{A pair of vertices $u,v\in V$, $\eps$, $\xi$.}
    \Output{An approximation $\hat{E}(\{u,v\})$ of $|E(\{u,v\})|$.}
	
	Define $k = 12\log(2/\xi)/(\eps^2)$.

    Call the oracle $\ONTWO$ $k$ times on $(u,v)$, and let $\hat{\alpha}$ be the fraction of returned edges that were $\{u,v\}$.

    Return $\hat{E}(\{u,v\}):=2\Delta_{\{u,v\}}(\{u\})\cdot \frac{1}{1+\hat{\alpha}}$.
 \caption{Approximating $|E(\{u,v\})|$}
\end{algorithm}

Note that this algorithm makes $k = O(\frac{\log(1/\xi)}{\eps^2})$ queries.

\begin{lemma}
    With probability at least $1-\xi$, $\hat{E}(\{u,v\})$ is an approximation of $|E(\{u,v\})|$ to within a factor of $(1 \pm \eps)$.
\end{lemma}
\begin{proof}

    Let $\alpha := \frac{|E\cap \{u,v\}|}{|E(\{u,v\})|}$ be the fraction of hyperedges that are $\{u,v\}$. The algorithm runs a Monte Carlo simulation to approximate $\alpha$ by the ratio $\hat{\alpha}$. In order to prove concentration of $\hat{\alpha}$ around $\alpha$, let $k'$ be the total number of $\{u,v\}$ edges returned, and observe that $k'$ is the sum of $k$ independent Bernoulli random variables each having probability equal to $\alpha$. By Chernoff bound, $\Pr[|k' - \alpha k| > \eps k/2]\leq 2\exp(-\alpha k \eps^2/12\alpha) \leq 2\exp(-k \eps^2/12) = 2\exp(\log(\xi/2)) = \xi$. Therefore with probability at least $1-\xi$, $|\hat{\alpha} - \alpha| \leq \eps/ 2$. This implies that $\frac{1}{1+\hat{\alpha}}\in \frac{1}{1+\alpha \pm \eps/2} \subseteq \frac{1}{(1 \pm \eps/2)(1+\alpha)}$. Finally, we use that $\frac{1}{(1\mp \eps/2)}\subseteq (1\pm \eps)$ to conclude that $\frac{1}{1+\hat{\alpha}}\in \frac{1\pm \eps}{1+\alpha}$, so 
	\[\frac{2\Delta_{\{u,v\}}(\{u\})}{1+\hat{\alpha}}\in (1\pm \eps)\frac{2\Delta_{\{u,v\}}(\{u\})}{1+\alpha} = (1\pm \eps)|E(\{u,v\})|.\]

\end{proof}


We now describe an algorithm to sample a random edge from $\delta(S)$, simulating a response to $\OED$. We first approximate the size of $E(\{u,v\})$ for each pair of vertices $u\in S$ and $v \in \bar{S}$. Then we sample a pair of $u,v$ with probability proportional to $\card{E(\{u,v\})}$, sample an edge in $E(\{u,v\})$, and then decide whether we keep it or not with probability proportional to its size. If we decide not to pick the edge, we repeat the whole process again.

 \begin{algorithm}[H]\label{alg:sample}
\SetAlgoLined
	\SetKwInOut{Input}{Input}\SetKwInOut{Output}{Output}

	\Input{A subset $S\subseteq V$}
	\Output{An edge $e\in \delta(S)$}
        For each pair of vertices $u,v$ such that $u \in S$ and $v \in \bar{S}$, call Algorithm~\ref{alg:pair} with $\xi = 1/n^{20}$, and let $\hat{E}(\{u,v\})$ be the output\;
        Sample a pair of vertices $(u,v)\in S\times \bar{S}$ with probability proportional to $\hat{E}(\{u,v\})$\;
		Use the oracle $\ONTWO$ to sample an edge $e$ in $E(\{u,v\})$\;
        With probability $\frac{1}{|e\cap S|\cdot |e\cap \bar{S}|}$, return	$e$. Otherwise go to Step 2.
	
 \caption{Sampling an edge in $\delta(S)$}
\end{algorithm}

\begin{lemma}
    With probability at least $1 - 1/n^{-10}$, Algorithm~\ref{alg:sample} samples each edge in $\delta(S)$ gets with probability $\frac{1 \pm \eps}{\card{\delta(S)}}$. The expected running time is $\tilde{O}(n^2/\eps^2)$.
\end{lemma}
\begin{proof}
    We first condition on the $|S|\cdot |\bar{S}|\leq n^2$ events that for each pair $u, v$ with  $u\in S$ and $v\in \bar{S}$, the estimate $\hat{E}(\{u,v\})$ was indeed in $(1\pm \eps)\cdot |E(\{u,v\})|$, which happens with probability at least $1 - n^2 \xi > 1- 1/n^{-10}$. Now fix an edge $e \in \delta(S)$. The probability that it was sampled at a particular iteration of Algorithm~\ref{alg:sample} is
    \[ \sum_{u\in S\cap e, v\in \bar{S}\cap e}\frac{\hat{E}(\{u,v\})}{\sum_{(u',v') \in S \times \bar{S}}\hat{E}(\{u',v'\})}\cdot \frac{1}{|E(\{u,v\})|}\cdot \frac{1}{|e\cap S|\cdot |e\cap \bar{S}|} \]
    \[ \in \frac{1}{\sum_{(u',v') \in S \times \bar{S}}\hat{E}(\{u',v'\})}\sum_{u\in S\cap e, v\in \bar{S}\cap e}\frac{(1\pm \eps)}{|e\cap S|\cdot |e\cap \bar{S}|} = \frac{(1\pm \eps)}{\sum_{(u',v') \in S \times \bar{S}}\hat{E}(\{u',v'\})}\]

That is, the probability of sampling each edge at any given iteration of Algorithm~\ref{alg:sample} is within $(1\pm \eps)$ of every other edge. Therefore the probability of sampling each edge is within a factor of $(1\pm \eps)$ of every other edge.

    Step $1$ calls Algorithm~\ref{alg:pair} $O(n^2)$ times, so the running time is $\tilde{O}(n^2/\eps^2)$. At step $4$, the probability that we keep the edge and finish the algorithm is at least $1/n^2$, so the expected number of iterations through step 2 to 4 is at most $n^2$. So the total running time on step 2 to 4 is $\tilde{O}(n^2)$ in expectation.
\end{proof}

\begin{proof}[Proof of Theorem~\ref{thm:neighbor}]
    We run Algorithm~\ref{alg:pesudo}, but each time it calls $\OED$, we instead run Algorithm~\ref{alg:sample} twice. With high probability, each time we simulate $\OED$ by Algorithm~\ref{alg:sample}, the probability of any edge in the cut being sampled is within a $(1\pm \eps)$ factor of the uniform distribution. Denote by $q'_e$ be the probability that an edge $e$ is sampled by this algorithm, and let $q_e$ be the probability that the edge $e$ is sampled in Algorithm~\ref{alg:pesudo}. We have $q'_e \in 2(1 \pm \eps) q_e$, which is larger than $p_e$ the probability of sampling an edge in Theorem~\ref{thm:kk}. Also we cannot directly compute $q'_e$, but we can approximate it to within a factor of $(1 \pm \eps)$, which only adds another $(1 \pm \eps)$ factor to the approximation achieved by the cut sparsifier.

    Since the number of calls to $\OED$ oracle in Algorithm~\ref{alg:pesudo} is $\tilde{O}(n^4/\eps^2)$. 
\end{proof}


==> _ <==
\section{Lower Bounds}
\subsection{$\OVA$ and $\ONONE$ are not Enough}
In this section, we prove that only with $\OVA$ and $\ONONE$, it is not possible to find a proper $(1 \pm \eps)$-approximate cut sparsifier with polynomial number (in $n$) of queries.

\begin{lemma}
	There is no polynomial time algorithm that can use $\OVA$ and $\ONONE$ to construct a $(1\pm \eps)$-approximate sparsifier of $H$ with probability more than $1/2+\epsilon$
\end{lemma}

\begin{proof}
	Suppose the runtime of the algorithm is bounded by some polynomial $f(n)$. We construct two graphs $H_1=(V\cup V', E_1)$ and $H_2 = (V\cup V', E_2)$ with $|V| = |V'| = n$ such that any algorithm only accesses to $\OVA$ and $\ONONE$ cannot distinguish these two graphs but there exists a cut such that there is no common edge accross the cut.

	Let $u,v\in V$ and $u',v'\in V'$ be some arbitrary vertices. Let $E=2^V\cup 2^{V'}$ be the union of the complete hypergraphs on $V$ and $V'$. We define $E_1$ as $E$ along with the edges all possible edges of size two among $\{u,v,u',v'\}$. We define $E_2$ as $E$ along with all possible edges of size $3$ among $\{u, v, u', v'\}$. It is easy to verify that for any cut, the number of edges in $E_1$ crossing the cut equals the number of edges in $E_2$ crossing the cut. So any cut size query has the same answer in $H_1$ and $H_2$.

	Additionally, the algorithm can make at most $f(n)$ calls to $\ONONE$. But the probability that a uniform random edge containing a fixed vertex is not in $E$ is at most $3/2^n$. Using a union bound over all $f(n)$ queries, we get that for both hypergraphs, with probability at least $1-2f(n)/2^n$, all of the sampled edges are in $E$.

	Since $2f(n)/2^n < \epsilon$ for large $n$, this implies that conditioned on the event that all sampled edges are in $E$. Note that conditioned on this event, the algorithm cannot. Therefore there is nonzero probability that the output of the algorithm is both a sparsifier of $H_1$ and $H_2$, which is a contradiction, because every sparsifier of $H_2$ must have the hyperedge $\{u, v, v'\}$, which is not present in $H_1$.


\end{proof}

